In defense of parameter sharing for model-compression

When considering a model architecture, there are several ways to reduce its memory footprint. Historically, popular approaches included selecting smaller architectures and creating sparse networks through pruning. More recently, randomized parameter-sharing (RPS) methods have gained traction for model compression at start of training. In this paper, we comprehensively assess the trade-off between memory and accuracy across RPS, pruning techniques, and building smaller models. Our findings demonstrate that RPS, which is both data and model-agnostic, consistently outperforms/matches smaller models and all moderately informed pruning strategies, such as MAG, SNIP, SYNFLOW, and GRASP, across the entire compression range. This advantage becomes particularly pronounced in higher compression scenarios. Notably, even when compared to highly informed pruning techniques like Lottery Ticket Rewinding (LTR), RPS exhibits superior performance in high compression settings. This points out inherent capacity advantage that RPS enjoys over sparse models. Theoretically, we establish RPS as a superior technique in terms of memory-efficient representation when compared to pruning for linear models. This paper argues in favor of paradigm shift towards RPS based models. During our rigorous evaluation of RPS, we identified issues in the state-of-the-art RPS technique ROAST, specifically regarding stability (ROAST's sensitivity to initialization hyperparameters, often leading to divergence) and Pareto-continuity (ROAST's inability to recover the accuracy of the original model at zero compression). We provably address both of these issues. We refer to the modified RPS, which incorporates our improvements, as STABLE-RPS.

==> main_paper/introductions.tex <==
\section{Introduction}
% what are we trying to figure out.
Model architecture design in Machine learning has been an important area of research as it affects not only the accuracy of the downstream task but also resource requirements of training and deployment.  Given a task, models are usually designed using domain expertise often augmented with neural architectural search over standard layers. Lottery Ticket Hypothesis (LTH) was one of the first papers, which showed the inefficient usage of parameters in models built from standard neural network components. LTH and its follow-up works have shown that given a model at the start of training, they can derive lighter models (alternatively models compressed at start), using pruning techniques, which can be trained to the same accuracy using same amount of time. With this, various pruning techniques such as \mg, \snip, \grasp, \synflow, etc. have emerged to prune standard models at the start of training.  Given the increasing popularity of pruning approaches, we ask the question \textit{``Is pruning parameters the correct way to obtain the best memory-efficient architecture (one that gives the best memory-accuracy trade-off)"}

% RPS vs pruning. rps is better - why?
In this paper, we consider Parameter Sharing as an alternative to pruning in order to obtain memory-efficient architecture from a given model architecture.  We rigorously test memory-accuracy curves for different pruning methods and Randomized parameter sharing (\rps) (data and model agnostic parameter sharing) on different models and datasets in computer vision which are historically used to evaluate pruning methods. We find that RPS not only outperforms {\rand } but also consistently outperforms moderately informed pruning methods such as \mg, \snip, {\grasp } and \synflow, especially in high compression regimes. While {\rps } is inferior to the highly informed and computationally expensive pruning technique of Lottery Ticket Rewinding (\ltr) in low compression region, it surprisingly is significantly better than {\ltr } in high compression region. This highlights the inherent capacity advantage that RPS enjoys as compared to pruning - given a parameter budget, parameter shared model is better at preserving the function than a sparse model. Due to this capacity disadvantage, even a highly informed pruning (like LTR) is worse than vanilla uninformed parameter sharing method. We theoretically establish this advantage in section \ref{sec:theory} for linear models. While we restrict our attention to RPS which is model and data-agnostic method, our results encourage  research in informed parameter sharing based models to achieve even better memory-accuracy tradeoff.

%Improvemnets in ROAST.
In our endeavor to rigorously evaluate {\rps }, we use the SOTA RPS scheme of {\roast } and find two major issues in {\roast } (1) stability: The {\roast } with its global-memory-sharing introduces a new hyper-parameter of initialization standard-deviation of the {\roast } array. This standard deviation determines the different multiplicative factors used for each component. We find that it is important to choose a standard-deviation which keeps the multiplicative factors in check. Any extreme choice such as low standard-deviation will blow up multiplicative factors causing divergence and high standard-deviation will suppress multiplicative factors causing slow learning. We provide a gradient scaling scheme that provable improves the stability of the training and removes its sensitivity to initialization standard-deviation. (2) pareto-continuity : {\roast } cannot recover the accuracy of full model when compression is set to $1\times$ (no compression). This is a desirable property for any compression method and pruning achieves this naturally. We propose a different mapping function which maintains the cache-efficient memory coalescing, obtains the optimal number of collisions and also has the pareto-continuity property - when compression is set to $1\times$ there is no collision thus the model with {\rps } is equivalent to full model. {\roast } along with improvements in gradient updates and mapping function is collectively referred as {\roastpp} in the paper.

We make the following contributions,
\begin{itemize}[nosep, leftmargin=*]
\item We identify and elucidate the shortcomings of existing state-of-the-art parameter-sharing method {\roast } with regard to issues related to stability and Pareto-continuity.
\item We introduce a set of enhancements that provably and demonstrably rectify the stability and Pareto-continuity problems within {\roast }. These enhancements are collectively referred to as {\roastpp }.

\item We conduct a comprehensive evaluation of {\roastpp } in comparison to pruning at initialization methods such as (1) uninformed pruning: {\rand }, (2) Moderately informed pruning : {\mg }, {\snip }, {\synflow }, and {\grasp }, and (3) highly informed pruning : Lottery Ticket Rewinding ({\ltr }). Our evaluation is performed on benchmark vision tasks that have historically been used to assess pruning techniques. Remarkably, our findings consistently demonstrate that {\roastpp } either matches or surpasses the performance of uninformed and moderately informed pruning methods. Notably, this superior performance holds true, especially in high compression scenarios where {\roastpp } beats even highly informed pruning like {\ltr } with significant margins. This is a noteworthy result considering that ROAST++ relies solely on a random (and thus uninformed) hash function, while other methods attempt to leverage various properties to intelligently prune the model during initialization. 

\item We provide theoretical insights to explain why compressed models based on parameter sharing exhibit superior capacity compared to pruned models.


\end{itemize}
The rest of this paper is organized as follows. We briefly discuss the development in model compression at start of training and explain how {\roast } works in section \ref{sec:background}. In section \ref{sec:stability} and \ref{sec:pareto}, we describe the issues associated with {\roast } and fixes which we collectively call {\roastpp }. In section \ref{sec:tradeoff} we discuss our rigorous evaluation of memory-accuracy trade-off followed by discussion on future directions in section \ref{sec:discussion}.

==> main_paper/stability.tex <==
\subsection{Stability of optimization}
ROAST introduces additional hyper-parameter - initialization standard deviation which is used to initialize the ROAST array. This determines the scaling factors used for each of the modules. The effect of this hyper-parameter is not discussed in their paper. However, we find that optimization convergence and generalization performance is very sensitive to this hyperparameter. The effects of not choosing this hyper-parameter can lead to convergence to poor generalization performance also marked by large norms of the observed solutions. It can even lead to  divergence of optimization leading to no-learning in the system. We propose a gradient scaling mechanism that removes the sensitivity to this hyper-parameter - reducing hyper-parameter tuning, giving reasonable norms of solutions and stable (often near optimal if not optimal) generalization performance. 



==> main_paper/subspace_choice.tex <==
\section{In defense of Parameter-Sharing paradigm over other options} \label{sec:theory}
Most model compression methods such as pruning, quantization, distillation are focused on inference benefits. Recently, there have been efforts to reduce the training time resources for model training. This paper focuses on training time model compression. Consider the following question : \textit{Given a fixed memory budget say $M$, what is the best model you can train}. A few tools from literature at our disposal are - build architectures that fit the memory, take a sparse subnetwork from a bigger model and use low-precision ( a naive version of quantization) parameters to save memory. The low-precision method can be applied in conjunction with any other compression methods and usually give a factor improvement of memory usage out of the box. Generally, smaller models for a dataset train to lower quality as compared to larger models. However, a series of papers on LTH highlighted that larger architecture can be sparsified to obtain a smaller model, and that this sparse model provides better memory accuracy trade-off. LTH uses iterative magnitude pruning and rewinding to find this sparse subnetwork. This process is costly and generally requires training models (larger than the memory budget) multiple times. Since then, there has been efforts to reduce the cost of finding the sparse subnetwork. 

Training a sparse subnetwork of a larger model is essentially looking for solution to the larger model in a \textit{co-ordinate} aligned subspace of the original solution space. This paper asks the question \textit{"is co-ordinate aligned subspace a good subspace to find a low memory solution?"}. Recently, a different method has been proposed to reduce the memory footprint of the model which is based on parameter sharing. Training a large model that shares parameters from a small memory repository is equivalent to searching for a solution to the larger model in a subspace that is defined by the column-space of the mapping matrix. The subspaces of parameter sharing based methods such as ROAST++ are non-aligned. This paper finds that non-aligned sub spaces are better than aligned-subspaces and provides better memory-accuracy trade-off.

In our first experiment, we evaluate parameter sharing method of ROAST++ against different types of pruned models on three standard datasets generally used to evaluate pruning quality - CIFAR-10, CIFAR-100 and  Tiny-Imagenet on three types of pruning methods 
\begin{enumerate}
    \item \rand (random pruning): This is the real \textbf{head to head} comparison between ROAST based randomly drawn non-aligned subspace which is uninformed of the initialization or the data. \rand will prune the network randomly and essentially select a random aligned subspace. 
    
    \item \textbf{Moderately Informed pruning}: Various pruning at start methods have been proposed using information from either initialization ( \mg ) and from gathering gradient / hessian information using data on full model ( \synflow, \snip, \grasp ). As pointed in \synflow paper, these pruning methods can be improved if the pruning is done iteratively . So we use them with their iterative variants. ROAST is not privy to this information which tips the scale in favor of pruning methods. 
    
    \item \textbf{Highly Informed pruning}: As a representative of this method, we choose Lottery Ticket Rewinding which applies the iterative magnitude pruning with rewinding the weights. We use rewinding to 500it in our experiments. This represents the best of what aligned sub-spaces may potentially achieve in terms of accuracy memory trade-off. Note that generally these methods are prohibitive and not practical.
    
\end{enumerate}


We make the following observations from the above plots,
\begin{itemize}
    \item In a head-to-head comparison of uniformed choices of subspaces, ROAST++ outperforms \rand at all levels of compression. This shows a random choice of aligned subspace is a poor choice than a random choice of non-aligned sub spaces (restricted to those obtained by ROAST hashing)
    \item Even a random and uninformed non-aligned subspace is competitive with the best of all pruning methods (which changes across compression / datasets) (in low compression regime) and significantly better than moderately informed pruning techniques such as \mg, \rand, \snip, \synflow. 
    \item A highly informed pruning method such as one used in LTR is also worse in high compression regimes when compared to a naive randomly selected non-aligned subspace. 
\end{itemize}
The above observations show that the choice of aligned-subspace is inferior to the non-aligned subspaces. Even a highly informed aligned subspace at high compression is worse for finding a solution when compared to naively chosen random non-aligned subspace. Firstly, this shows that non-aligned subspaces are the state of the art memory-reduction technique when memory budgets are low. Secondly, research in how to select non-aligned subspaces in an informed manner seems promising to improve the state-of-the-art in memory-budgeted model training.

The question then arises as to why parameter sharing works better than pruning approaches? In order to investigate this further, we run a full model fine tuning from the solutions obtained in the respective subspaces. We make the following observations and comments,
\begin{itemize}
    \item while ROAST almost always obtains a solution at par with full model trained from scratch, other methods obtain solutions that are of inferior quality
    \item The cases which have experienced layer-collapse  do not recover during fine-tuning. This is expected as the gradients are zeros in this computational graph. Even if we initialize the zeros with noise with small standard deviation, the situation does not improve much. Adding higher noise is a solution, but the result is hard to interpret as we do not have the answer to the question "how much noise will make the point stay in the area around the starting point".
    \item Methods such as \mg, \snip, \synflow, and \grasp  show that full model fine tuning falls short of the full model (trained from scratch) accuracy with significant margins. They can only improve a bit over subspace solutions. This shows that an informed aligned subspace lands in a area of solution space that has bad local minima. 
    \item \rand shows interesting results. For subspaces that have not experienced layer collapse, \rand  with full fine tuning recovers the full model (trained from scratch) accuracy. This implies that moderately informed pruning does a chooses subspace that have good local solutions but might be inside area which has a bad local minima in the full space. 
    \item However, \rand is more susceptible to layer collapse and bad in-subspace minimas making it a bad option for memory reduction.
    \item Moderately informed pruning methods are bad if we plan to increase memory budget in the future and fine tune the model. 
    \item On both these aspects - in-subpsace solutions and full-space fine-tuning, ROAST is superior to uninformed \rand and informed \synflow, \mg, \snip, and \grasp
\end{itemize}

Further investigating the cause of loss of accuracy in pruning methods, we find that there are parts of the model that cannot be recovered during fine tuning. This is clear from the evolution of sparsity shown in figure \ref{fig:2}

\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[scale=0.40]{finetune/finetuning.cifar10.1.0.png}
        
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[scale=0.40]{finetune/sparsity.cifar10.synflow.1.0.png}
    \end{subfigure}
        \caption{[LEFT]Evolution of accuracies during full fine tuning for starting from 10x compressed models.[RIGHT] Sparsity evolution with iterations. The sparsity decreases rapidly in first few iterations but plateaus quickly without reaching 1.0 for most layers. This shows partial-model-collapse that happens in these subspaces. some dimensions are not reachable to be updated and thus utilized.}    \label{fig:2}
\end{figure}


\subsection{Theoretical discussion around model compression}
Analysing the deep learning in its full glory has always been a theoretical challenge. How do we, then, analyse the effect of aligned vs. non-aligned subspaces on model solutions? In this section, we use different settings traditionally used in literature. In this section we not only search for theoretical understanding of why non-aligned subspaces are better, but also to understand what tools and settings can and cannot distinguish between the two choices of subspaces. We start with a simple settings,
\subsubsection{Dimensionality reduction under subspace projection.}

==> tables/cifar10-stability.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{[CIFAR-10 with RESNET-20]Sensitivity of ROAST to initialization hyper parameter and robustness of ROAST++ to this hyperparameter} \label{fig:cifar10-stability}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c||ccccc||ccccc|}
\hline
\rowcolor[HTML]{FFFFFF} 
\textit{}                                       &                                 & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Accuracy}                                                                                                                                                                                                                                                                                 & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Solution Norms}                                                                                                                                                                                                                                                                         \\ \hline
\rowcolor[HTML]{FFFFFF} 
sparsity                                        & init stdev $\rightarrow$        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}} & {\color[HTML]{333333} 10}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}} & {\color[HTML]{333333} 10}  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \cellcolor[HTML]{FFFFFF}ROAST   & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}10.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFE800}86.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}91.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFE00}90.4}                     & \cellcolor[HTML]{FFB900}79.4 & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}639}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{05FA00}64}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFF00}27}                       & \cellcolor[HTML]{7CFF00}40 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}25}    & \cellcolor[HTML]{FFFFFF}ROAST++ & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}91.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}91.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}91.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}91.2}                     & \cellcolor[HTML]{00FF00}91.4 & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56}                       & \cellcolor[HTML]{01FE00}56 \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \cellcolor[HTML]{FFFFFF}ROAST   & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}10.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFE400}81.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}87.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{08FF00}86.4}                     & \cellcolor[HTML]{FFC300}77.3 & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1159}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{1CE300}110}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{ECFF00}29}                       & \cellcolor[HTML]{7FFF00}40 \\ \cline{2-12} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}90}    & \cellcolor[HTML]{FFFFFF}ROAST++ & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}87.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}87.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}87.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}87.0}                     & 87.4                         & \multicolumn{1}{c|}{\cellcolor[HTML]{01FF00}53}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}53}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}53}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{01FF00}53}                       & \cellcolor[HTML]{01FF00}53 \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \cellcolor[HTML]{FFFFFF}ROAST   & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}10.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFF800}69.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}75.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{25FF00}74.2}                     & \cellcolor[HTML]{FFD400}66.8 & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}2506}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{609F00}248}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{77FF00}41}                       & \cellcolor[HTML]{64FF00}43 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99}    & \cellcolor[HTML]{FFFFFF}ROAST++ & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}75.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}75.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}75.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}74.9}                     & \cellcolor[HTML]{00FF00}75.1 & \multicolumn{1}{c|}{\cellcolor[HTML]{32FF00}48}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{37FF00}47}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{34FF00}48}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{33FF00}48}                       & \cellcolor[HTML]{31FF00}48 \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \cellcolor[HTML]{FFFFFF}ROAST   & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}10.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}10.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{63FF00}53.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}56.0}                     & \cellcolor[HTML]{95FF00}52.1 & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F60900}549}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{1FE000}116}                      & \cellcolor[HTML]{74FF00}41 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99.99} & \cellcolor[HTML]{FFFFFF}ROAST++ & \multicolumn{1}{c|}{\cellcolor[HTML]{72FF00}52.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{8CFF00}52.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{49FF00}53.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{0BFF00}54.8}                     & \cellcolor[HTML]{95FF00}52.1 & \multicolumn{1}{c|}{\cellcolor[HTML]{50FF00}45}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{4DFF00}45}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{4AFF00}45}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{41FF00}46}                       & \cellcolor[HTML]{4BFF00}45 \\ \hline
\end{tabular}
}
\end{table}

==> tables/cifar100-stability.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\caption{[CIFAR-100 with VGG11]Sensitivity of ROAST to initialization hyper parameter and robustness of ROAST++ to this hyperparameter}\label{fig:cifar100-stability}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\resizebox{\textwidth}{!}{
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c ||cc
>{\columncolor[HTML]{00FF00}}ccc||ccc
>{\columncolor[HTML]{00FF00}}c 
>{\columncolor[HTML]{00FF00}}c |}
\hline
\textit{}                                       &                          & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Accuracy}                                                                                                                                                                                                                                                                                                      & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}Solution Norms}                                                                                                                                                                                                                                                                                                \\ \hline
sparsity                                        & init stdev $\rightarrow$ & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-3}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-2}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1e-1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 1}} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 10} \\ \hline
\cellcolor[HTML]{FFFFFF}                        & ROAST                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{21FF00}67.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{15FF00}67.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{E4FF00}63.6}                     & \cellcolor[HTML]{FF0000}19.8                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}8k}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}659}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}73}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}67}                       & 75                                                \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}25}    & ROAST++                  & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}68.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}68.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}68.9}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}68.2}                     & \cellcolor[HTML]{00FF00}68.6                      & \multicolumn{1}{c|}{\cellcolor[HTML]{0AF500}115}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{0AF500}115}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{0AF500}115}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{0AF500}115}                      & \cellcolor[HTML]{02FD00}109                       \\ \hline
\cellcolor[HTML]{FFFFFF}                        & ROAST                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}38.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}66.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFE900}62.8}                     & \cellcolor[HTML]{FF0000}19.9                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}8k}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}57}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}106}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}68}                       & 75                                                \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}90}    & ROAST++                  & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}65.8}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}66.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}66.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}66.0}                     & \cellcolor[HTML]{00FF00}66.3                      & \multicolumn{1}{c|}{\cellcolor[HTML]{0DF200}117}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{0DF200}117}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{0DF200}117}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{0DF200}117}                      & \cellcolor[HTML]{0CF300}116                       \\ \hline
\cellcolor[HTML]{FFFFFF}                        & ROAST                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{EAFF00}54.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{0AFF00}57.1}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F9FF00}54.4}                     & \cellcolor[HTML]{FF0000}20.2                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}14k}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1741}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{798600}192}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}70}                       & 75                                                \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99}    & ROAST++                  & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}57.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}57.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}57.3}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}57.4}                     & \cellcolor[HTML]{00FF00}58.2                      & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}94}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}94}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}93}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}94}                       & 93                                                \\ \hline
\cellcolor[HTML]{FFFFFF}                        & ROAST                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1.0}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFB00}17.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}25.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{10FF00}24.7}                     & \cellcolor[HTML]{FFEF00}17.1                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}5595}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}675}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{14EB00}122}                      & 72                                                \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99.99} & ROAST++                  & \multicolumn{1}{c|}{\cellcolor[HTML]{39FF00}23.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{3DFF00}23.4}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{33FF00}23.7}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{3AFF00}23.5}                     & \cellcolor[HTML]{36FF00}23.6                      & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}83}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}85}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}84}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}84}                       & 85                                                \\ \hline
\end{tabular}
}
\end{table}

==> tables/temp.tex <==
\begin{table}[h]
\centering
\caption{CIFAR-100(VGG11) sensitivity of roast to initialization standard deviation}
\begin{tabular}{|c|crrrrr|}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{Accuracy}                               & \multicolumn{6}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Initialization standard deviation}}                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\textbf{sparsity}                               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{scale}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.001}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.01}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 10}} \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1.00}                         & \multicolumn{1}{r|}{\cellcolor[HTML]{21FF00}67.24}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{15FF00}67.47}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{E4FF00}63.58}                    & \cellcolor[HTML]{FF0000}19.77                                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}25.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}68.12}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}68.07}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}68.86}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}68.17}                    & 68.58                                                                  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}38.73}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1.00}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}65.97}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE900}62.76}                    & \cellcolor[HTML]{FF0000}19.94                                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}90}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}65.60}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}66.52}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}66.05}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}65.98}                    & 66.34                                                                  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1.00}                         & \multicolumn{1}{r|}{\cellcolor[HTML]{EAFF00}54.54}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{0AFF00}57.05}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{F9FF00}54.38}                    & \cellcolor[HTML]{FF0000}20.24                                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}57.47}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}57.38}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}57.30}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}57.42}                    & 58.16                                                                  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1.00}                         & \multicolumn{1}{r|}{\cellcolor[HTML]{FFB700}17.64}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}25.45}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}24.66}                    & \cellcolor[HTML]{FFB100}17.23                                          \\ \cline{2-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{66FF00}23.70}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{92FF00}23.38}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{6CFF00}23.65}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{88FF00}23.45}                    & \cellcolor[HTML]{77FF00}23.57                                          \\ \hline
\end{tabular}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[h]
\centering

\caption{CIFAR-10(RESNET20) sensitivity of roast to initialization standard deviation}
\begin{tabular}{|c|crrrrr|}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{Accuracy}                               & \multicolumn{6}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Initialization standard deviation}}                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\textbf{sparsity}                               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{scale}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.001}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.01}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 10}} \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}10.00}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE800}86.91}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}91.50}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FFFE00}90.40}                    & \cellcolor[HTML]{FFB900}79.39                                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}25.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}91.40}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}91.20}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}91.31}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}91.20}                    & 91.38                                                                  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}10.00}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFE400}81.87}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}87.23}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{08FF00}86.36}                    & \cellcolor[HTML]{FFC300}77.31                                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}90}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}87.29}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}87.34}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}87.35}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}87.01}                    & 87.38                                                                  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}10.00}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FFF800}69.64}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}75.47}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{25FF00}74.16}                    & \cellcolor[HTML]{FFD400}66.81                                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}75.17}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}75.83}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}75.21}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}74.91}                    & 75.15                                                                  \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}10.00}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}10.00}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{63FF00}53.08}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}56.03}                    & \cellcolor[HTML]{95FF00}52.09                                          \\ \cline{2-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{72FF00}52.77}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{8CFF00}52.27}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{49FF00}53.57}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{0BFF00}54.80}                    & \cellcolor[HTML]{95FF00}52.08                                          \\ \hline
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\centering
\caption{CIFAR100(VGG11) Solution norms}
\begin{tabular}{|c|crrrrr|}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{Accuracy}                               & \multicolumn{6}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Norms of solutions}}                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\textbf{sparsity}                               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{scale}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.001}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.01}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 10}} \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}8221.6}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}658.7}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}72.8}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}67.4}                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                          \\ \cline{2-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}25.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                             & \multicolumn{1}{r|}{\cellcolor[HTML]{03FC00}114.9}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{03FC00}115.0}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{03FC00}115.1}                    & \cellcolor[HTML]{00FF00}109.3                                          \\ \hline
\rowcolor[HTML]{00FF00} 
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}7965.4}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}57.0}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}105.8}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}67.6}                     & 74.9                                                                   \\ \cline{2-7} 
\rowcolor[HTML]{04FB00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}90}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{04FB00}117.3}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{04FB00}117.0}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{04FB00}117.0}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{04FB00}116.8}                    & \cellcolor[HTML]{03FC00}116.1                                          \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}14428.6}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}1741.4}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{2ED100}192.3}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}70.3}                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}}                          \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}93.7}                         & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}93.6}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}93.5}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}93.5}                     & 93.4                                                                   \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}3x$10^14$}                    & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}5595.0}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{FF0000}674.9}                      & \multicolumn{1}{r|}{\cellcolor[HTML]{07F800}122.1}                    & \cellcolor[HTML]{00FF00}72.0                                           \\ \cline{2-7} 
\rowcolor[HTML]{00FF00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}82.8}                         & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}84.7}                        & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}84.1}                       & \multicolumn{1}{r|}{\cellcolor[HTML]{00FF00}83.7}                     & 84.6                                                                   \\ \hline
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{CIFAR10(RESNET20) Solution norms}
\begin{tabular}{|c|cccccr|}
\hline
\rowcolor[HTML]{FFFFFF} 
\textbf{Accuracy}                               & \multicolumn{6}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{Solution Norms}}                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\rowcolor[HTML]{FFFFFF} 
\textbf{sparsity}                               & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{scale}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.001}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.01}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 0.1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 1}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 10}} \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}638.9}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{05FA00}63.5}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFF00}27.4}                     & \cellcolor[HTML]{7CFF00}40.4                                           \\ \cline{2-7} 
\rowcolor[HTML]{01FE00} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}25.01} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56.4}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56.5}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56.2}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{01FE00}56.3}                     & 55.8                                                                   \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}1159.0}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{1CE300}110.4}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{ECFF00}29.4}                     & \cellcolor[HTML]{7FFF00}40.1                                           \\ \cline{2-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}90}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{c|}{\cellcolor[HTML]{01FF00}52.6}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}52.6}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{00FF00}52.6}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{01FF00}52.6}                     & \cellcolor[HTML]{01FF00}52.6                                           \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}2506.4}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{609F00}247.7}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{77FF00}40.9}                     & \cellcolor[HTML]{64FF00}42.7                                           \\ \cline{2-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99}    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{c|}{\cellcolor[HTML]{32FF00}47.7}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{37FF00}47.2}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{34FF00}47.5}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{33FF00}47.6}                     & \cellcolor[HTML]{31FF00}47.8                                           \\ \hline
\cellcolor[HTML]{FFFFFF}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST}           & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                          & \multicolumn{1}{c|}{\cellcolor[HTML]{FF0000}nan}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{F60900}548.9}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{1FE000}116.2}                    & \cellcolor[HTML]{74FF00}41.2                                           \\ \cline{2-7} 
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}99.99} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ROAST++}             & \multicolumn{1}{c|}{\cellcolor[HTML]{50FF00}44.7}                         & \multicolumn{1}{c|}{\cellcolor[HTML]{4DFF00}45.0}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{4AFF00}45.4}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{41FF00}46.2}                     & \cellcolor[HTML]{4BFF00}45.2                                           \\ \hline
\end{tabular}
\end{table}

==> text/app_exp1.tex <==
\section{Comprehensive evaluation of parameter sharing vs pruning at initialization.}
In this section, we first evaluate \textbf{ROAST++} based parameter sharing method against the spread of various pruning at initialization. We find that random non-aligned (restricted) subspace selected by \textbf{ROAST++} is always better than a random co-ordinate aligned subspace selected by random pruning. Moreover, non-aligned subspace chosen at random are better than even intelligently selected aligned subspaces (using methods such as $\mathrm{MAG}$, $\mathrm{GRASP}$, $\mathrm{SNIP}$, $\mathrm{SYNFLOW}$)

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\linewidth]{exp1/CIFAR-10(ResNet-20).png}    
    \end{subfigure}
    \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\linewidth]{exp1/CIFAR-100(VGG-11).png}    
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
    \includegraphics[width=\linewidth]{exp1/TINY-IMAGENET(RESNET-18).png}    
    \end{subfigure}
    \label{fig:enter-label}
\end{figure}

==> text/convergence_theory.tex <==
\section{Convergence of {\roast} and {\roastpp}} \label{app:convergence}

Consider a simple setting of $L$-smooth functions. Under ROAST, the recovery matrix can be decomposed into mapping matrix and scaling matrix. The sign can go inside the scaling matrix. 

Let the full model parameters be $\theta \in R^n$ and $\psi\in R^m$ be the roast array. We skip the permutation matrix here.

\begin{equation}
    \theta = \Lambda R \psi 
\end{equation}
where R=$n \times m$ matrix and $\Lambda$ is diagonal matrix with $\Lambda_{ii} = g(i)\lambda_i$

Consider a function $F$ with lipschitz constant $L_f$. Thus we have 

\begin{equation}
    || \nabla F(x) - \nabla F(y) ||_2 \leq L_f ||x - y||_2
\end{equation}
Under projection based parameter sharing we have 
\begin{equation}
    G(\psi) = F(\Lambda R \psi) 
\end{equation}
\subsection{ROAST}
Thus we have,
\begin{align}
    & || \nabla G(x) - \nabla G(y) ||_2 \\
    & = || \nabla F(\Lambda R x) - \nabla F(\Lambda R y) ||_2 \\
    & \leq L_f ||\Lambda R x - \Lambda R y||_2 \\
    & \leq \rho(\Lambda R) ||x - y||_2
\end{align}

where $\rho(M)$ is the max singular value of the matrix M.  Thus, $L_g = L_f \rho(\Lambda R)$ is the lipschitz constant of $G(\psi)$.
\paragraph{tightness of $L_g$}
Given a function $F$, $L_f$ is tight if there exist a pair $x,y$ which satisfy the equality. Let $L_f$ be the tight lipschitz constant. Now, for $G$, $L_g$ is tight if and only if $x = \Lambda R x'$ and $y = \lambda R y'$ for some $x'$ and $y'$. For a function $F$ for which the particular pair x and y lie in column space of $\Lambda R$ can be constructed. Thus, with limited information, $L_g$ is tight. 

\begin{equation}
    \rho(\Lambda R)^2 = \textrm{eigen-value} ( (\Lambda R)^\top (\Lambda R)) 
\end{equation}
\begin{equation}
    \rho(\Lambda R)^2 = \textrm{eigen-value} ( R^\top \Lambda^2 R) 
\end{equation}
Note that under parameter shairng $\mathcal{S} = (R^\top \Lambda^2 R)$ is a diagonal matrix with
$\mathcal{S}[i,i] = \sum_{j, j=h(i)} \lambda_j^2$

Thus max eigen value is 
\begin{equation}
    \rho(\Lambda R) = \max_i \sqrt{ \sum_{j, i=h(j)} \lambda_j^2}
\end{equation}

The suggested stability range from gradient descent analysis with ROAST becomes
\begin{equation}
    \textrm{stability}(\eta) = \left(0, \frac{2}{L_g}\right) = \left(0, \frac{2}{\max_i \sqrt{ \sum_{j, i=h(j)} \lambda_j^2 } L_f } \right)
\end{equation}

\textit{Consider a function $F$, which is $L_f$ Lipschitz smooth, with $n$ parameters. Under RPS setup with RPS array of size $m$, hashing function $h$ and scaling factors $\lambda_1, \lambda_2 ,...,\lambda_n$. The stability range of gradient descent for learning rate goes from $(0, \frac{2}{L_f})$ for full model training to $\left(0, \frac{2}{\left( \max_{j=1}^m \sqrt{ \sum_{i=1, h(i) = j}^{i=n} \lambda_i^2 } \right) L_f}\right)$ for compressed model 
}

\subsection{Theory driven scaler in {\roastpp}}
Since f is lipschitz smooth, we have 
\begin{equation}
G(x_{t+1}) \leq G(x_t) + \langle \nabla G(x_t), x_{t+1} - x_t \rangle + L_g^2 || x_{t+1} - x_t ||_2^2    
\end{equation}


Under scaling the update is,
\begin{equation}
    x_{t+1} = x_{t} - \eta \Gamma \circ \nabla G(x_t)
\end{equation}

\begin{equation}
G(x_{t+1}) \leq G(x_t) + \langle \nabla G(x_t), - \eta \Gamma \circ \nabla G(x_t) \rangle + L_g^2 || \eta \Gamma \circ \nabla G(x_t) ||_2^2
\end{equation}

\begin{equation}
G(x_{t+1}) \leq G(x_t) - \eta \langle \nabla G(x_t),  \Gamma \circ \nabla G(x_t) \rangle + L_g^2 \eta^2 || \Gamma \circ \nabla G(x_t) ||_2^2
\end{equation}


\begin{align}
    & || \nabla g(x) - \nabla g(y) ||_2 \\
    & = || \Gamma  \nabla f(\Lambda R x) - \Gamma  \nabla f(\Lambda R y) ||_2 \\
    & \leq L_f ||\Gamma\Lambda R x - \Gamma\Lambda R y||_2 \\
    & \leq \rho(\Gamma\Lambda R) ||x - y||_2
\end{align}

\begin{equation}
    \rho(\Gamma \Lambda R) = \max_i \sqrt{ \sum_{j, i=h(j)} \gamma_i^2 \lambda_j^2}
\end{equation}

If
\begin{equation}
    \gamma_i = \sqrt{\frac{1}{\sum_{j, i = h(j)} \lambda_j^2} } 
\end{equation}

then,
\begin{equation}
    \rho(\Gamma \Lambda R) = 1
\end{equation}
Thus, the range of stability is,
\begin{equation}
    \textrm{stability}(\eta) = \left(0, \frac{2}{L_g}\right) = \left(0, \frac{2}{L_f}\right)
\end{equation}



==> text/simple_theory_1.tex <==
\section{Can Randomly chosen ROAST++ beat Random Pruning? : An anlaysis of linear models}

Consider a linear model of size $n$. Let the compressed model be of size $m$ where $n=mk$. For simplicity let us assume that $k$ is an integer. 


Let the true model be

\begin{equation}
    y = \sum_{i=1}^n \alpha_i x_i = \langle \alpha, x \rangle
\end{equation}

$x_is$ are normalized random variables with same standard deviation $\sigma$. Also, we assume that all the features are independent that is $Cov_{x \sim \mathcal{D}}(x_i, x_j) = 0$ if $i \neq j$.

\paragraph{Pruning at start / small model : } We will only choose $m$ weights which in turn selects $m$ inputs. 

Let the sampling matrix be $S \in \{0,1\}^{m \times n}$

\begin{equation}
    y_p = \sum_{i=1}^m \beta_{pi} x_{pi} = \langle \beta_p, S x \rangle
\end{equation}

\paragraph{ROAST++ (same sign):} We will use a repository of $m$ weights and use ROAST++ hashing to implement parameter sharing. This analysis assumes that ROAST assigns same sign inside the chunk.

Let $R \in \{ 0,1 \}^{n \times m}$ be the recovery matrix of ROAST++
\begin{equation}
    y_r =  \langle R \beta_s,  x \rangle  = \langle \beta_s, R^\top x \rangle 
\end{equation}

Let us look at the variances, 

\begin{equation}
    Var(y) = || \alpha ||_2^2 \sigma^2
\end{equation}

\begin{equation}
    Var(y_p) = || \beta_p ||_2^2 \sigma^2
\end{equation}

\begin{equation}
    Var(y_r) = Var( \sum_{i=1}^m \beta_{si} (x_{i1} + .... + x_{ik}) ) = k || \beta_s ||_2^2 \sigma^2 
\end{equation}

Now let us look at the covariance.

\begin{equation}
    Cov(y, y_p) = Cov ( \sum_{i=1}^n \alpha_i x_i, \sum_{i=1}^m \beta_{pi} x_{pi}) = \sum_{i=1}^m \alpha_{pi} \beta_{pi} \sigma^2 = \langle \beta, S \alpha \rangle  \sigma^2
\end{equation}


\begin{equation}
    Cov(y, y_r) = Cov ( \sum_{i=1}^n \alpha_i x_i, \sum_{i=1}^m \beta_{si} (x_{i1} + .... + x_{ik}) ))  = \sum_{i=1}^m (\beta_{si} (\alpha_{i1} + .... + \alpha_{ik})) \sigma^2 = \langle \beta, R^\top \alpha \rangle \sigma^2
\end{equation}

\begin{equation}
    \rho(y, y_r) = \frac{Cov(y,y_r)}{\sqrt{Var(y)}, \sqrt{Var(y_r)}} = \frac{\langle \beta_s, R^\top \alpha \rangle}{\sqrt{k} || \alpha ||_2 || \beta_s ||_2}
\end{equation}

\begin{equation}
    \rho(y, y_p) = \frac{Cov(y,y_p)}{\sqrt{Var(y)}, \sqrt{Var(y_p)}} = \frac{\langle \beta_p, S \alpha \rangle}{|| \alpha ||_2 || \beta_p ||_2}
\end{equation}

Note that 
\begin{equation}
    \max_x \frac{\langle a, x \rangle }{||x||} =  ||a||
\end{equation}
and is achieved when $x$ is aligned with $a$. Under learning we will reach this $\beta$s for both pruning/small mdoel and ROAST++.

Thus,

\begin{equation}
    \rho(y, y_r) = \frac{|| R^\top \alpha ||_2}{\sqrt{k} || \alpha ||_2 }
\end{equation}


\begin{equation}
    \rho(y, y_p) = \frac{|| S \alpha ||_2}{|| \alpha ||_2 }
\end{equation}


Let us take look at the square of correlation.

\begin{equation}
    \rho(y, y_p)^2  = \frac{\sum_{j=1}^n \alpha_j^2 \mathbf{1}_j }{ || \alpha ||^2 }
\end{equation}

\begin{equation}
    \mathbf{E}_S(\rho(y, y_p)^2)  = \frac{ || \alpha ||^2 \frac{1}{k} }{ || \alpha ||^2 } = \frac{1}{k}
\end{equation}

\begin{equation}
    \rho(y, y_r)^2  = \frac{ \sum_{i=1}^m \left( \sum_{j=1}^n \mathbf{1}_{i,j} \alpha_j \right)^2 }{ k || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \left( \sum_{j,k} \mathbf{E}(\mathbf{1}_{i,j,k} \alpha_j \alpha_k ) \right) }{ k || \alpha ||^2 } 
\end{equation}


\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \left( \left(\sum_{j=1}^n \mathbf{E}(\mathbf{1}_{i,j,j} \alpha_j^2 ) \right) + \left( \sum_{j \neq k} \mathbf{E}(\mathbf{1}_{i,j,k} \alpha_j \alpha_k \right)  \right) }{ k || \alpha ||^2 } 
\end{equation}


\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \frac{1}{m} ||\alpha||^2 + m \left( \sum_{j \neq k} \mathbf{E}(\mathbf{1}_{i,j,k} \alpha_j \alpha_k \right)   }{ k || \alpha ||^2 } 
\end{equation}


\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{1}{k} + \frac{  m \left( \sum_{j \neq k} \mathbf{E}(\mathbf{1}_{i,j,k} \alpha_j \alpha_k \right)   }{ k || \alpha ||^2 } 
\end{equation}
Assume that Roast is actually $R = PR$ where P is the permutation matrix.

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{1}{k} + \frac{  m \left( \sum_{j \neq k} \frac{1}{m}  \frac{(k-1)}{n-1} \alpha_j \alpha_k \right)   }{ k || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{1}{k} + \frac{  m \left( \frac{1}{m}  \frac{(k-1)}{n-1} \sum_{j \neq k } \alpha_j \alpha_k \right)   }{ k || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{1}{k} + \frac{  \left( (k-1) \sum_{j \neq k } \alpha_j \alpha_k \right)   }{ k (n-1) || \alpha ||^2 } 
\end{equation}


\begin{equation}
    \left(\sum \alpha_i \right)^2 = \sum \alpha_i^2 + 2 \sum_{j\neq k} \alpha_j \alpha_k
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{1}{k} + \frac{  \left( (k-1) (\sum \alpha_i)^2 - ||\alpha||^2 \right)   }{ 2 k (n-1) || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{1}{k} + \frac{  \left( (k-1) \right)   }{ 2 k (n-1)}  \left( 1 - \frac{(\sum \alpha_i)^2}{||\alpha||^2} \right)
\end{equation}

Thus,
\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \mathbf{E}_S(\rho(y, y_p)^2) + \frac{  \left( (k-1) \right)   }{ 2 k (n-1)}  \left( 1 - \frac{(\sum \alpha_i)^2}{||\alpha||^2} \right)
\end{equation}

Thus for linear models, randomly choosing the subspace via sampling or ROAST projections depends on the exact weights be approximated. Either can be better depending on exact $\alpha$.

\paragraph{ROAST++ (different sign):} We will use a repository of $m$ weights and use ROAST++ hashing to implement parameter sharing. This analysis assumes that ROAST assigns different sign inside the chunk which was originally proposed by the authors in \cite{roast}. Note that the variance of $y_r$ remains the same even with signs.

In this case, we will have ($g_i$ is the sign for  $i$)
\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \left( \sum_{j,k} \mathbf{E}(\mathbf{1}_{i,j,k} g_j g_k \alpha_j \alpha_k ) \right) }{ k || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \left( \sum_{j,k} \mathbf{E}(\mathbf{1}_{i,j,k} g_j g_k \alpha_j \alpha_k ) \right) }{ k || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \left( \left(\sum_{j=1}^n \mathbf{E}(\mathbf{1}_{i,j,j} \alpha_j^2 ) \right) + \left( \sum_{j \neq k} \mathbf{E}(\mathbf{1}_{i,j,k} g_j g_k \alpha_j \alpha_k \right)  \right) }{ k || \alpha ||^2 } 
\end{equation}

\begin{equation}
    \mathbf{E}_R(\rho(y, y_r)^2)  = \frac{ m \left( \frac{1}{m} || \alpha ||^2   \right) }{ k || \alpha ||^2 }  = \frac{1}{k} = \mathbf{E}_S(\rho(y, y_p)^2)
\end{equation}

So, in expectation, there is absolutely no advantage of random non-aligned subpsace (roast) over random aligned subspace (pruning).


\section{Can best ROAST++ beat best Pruning :  An analysis of linear models}
Unlike in previous analysis, where we assume that compression is oblivious to $\alpha$ (knowledge of $\alpha$ is only used in learning). In this analysis, we assume that we can choose the ROAST and pruning subspace with complete knowledge of the $\alpha$.


After learning, we get the following,

\begin{equation}
    \rho(y, y_r) = \frac{|| R^\top \alpha ||_2}{\sqrt{k} || \alpha ||_2 }
\end{equation}


\begin{equation}
    \rho(y, y_p) = \frac{|| S \alpha ||_2}{|| \alpha ||_2 }
\end{equation}

Now under best choice of $R$ and $S$, we need to evaluate the two correlations. Let us look at the sampling first,

Let $\alpha$ sorted in descending order by the magnitude of the individual co-ordinates be $(\alpha_1, \alpha_2, ... \alpha_n)$.
Then 
\begin{equation}
    \max || S \alpha ||_2^2 = \sum_{j=1}^m \alpha_j^2
\end{equation}

Under same notation, the roast matrix $R=PR$.
The max is

\begin{equation}
    \max || R^\top \alpha ||_2^2 = \sum_{j=0}^{m-1}(|\alpha_{jk+1}| + |\alpha_{jk+2}| + ... |\alpha_{jk+k}| )^2
\end{equation}

Note that even under best choice, there are cases where pruning would beat ROAST and ROAST would beat pruning. For example if $\alpha_1 = 1$ and rest all $\alpha_i$s are 0, pruning would be better. Whereas where the case where $\alpha_s = 1$, the ROAST would be better. 




So the next thing to look at is which of pruning vs ROAST covers most cases.

\subsection{special case of m=1 }
Consider a $\alpha$ drawn from a radially symmetric distribution (optionally normalized) Consider two sets of points. 
\begin{equation}
    \textrm{sparse-set} = \{ s | \exists i s[i] = \pm 1, \forall j \neq i s[j] = 0\}
\end{equation}

\begin{equation}
    \textrm{roast-set} = \{ r | \forall i , r[i] = \pm 1 \}
\end{equation}

\begin{equation}
    \max( \cos(\alpha, \textrm{sparse-set})) = max_i | \alpha[i] |
\end{equation}

\begin{equation}
    \max( \cos(\alpha, \textrm{sparse-set})) =  \frac{1}{\sqrt{k}}\sum_i |\alpha[i]|
\end{equation}
























\clearpage
\hline
Questionable
\hline

\section{Single parameter linear : Pruning vs Parameter sharing }

\paragraph{Setting} Consider a single neuron without activation. Let the data $x=(x_1, ..., x_k)$ come from a distribution $\mathcal{D}$. Also, we assume that for all $ i,j \in \{1,...,k\} , i \neq j, Cov_{x \sim \mathcal{D}}(x_i, x_j) = 0$. All variances and covariances are w.r.t $\mathcal{D}$ unless specified,

\begin{equation}
    y = \sum_{i=1}^k  \alpha_i x_i 
\end{equation}

We will compare,

\paragraph{1. pruning} choosing only one synapsis to be active and rest to be masked. WLOG, let us assume that we choose the first synapsis.

\begin{equation}
    y_p = \beta_p x_1
\end{equation}

\paragraph{2. parameter sharing:} choosing all synapsis to be active but sharing the same weight. 

\begin{equation}
    y_r = \beta_s \sum_{i=1}^k x_i
\end{equation}

We need to choose $\beta$ s. For effective modelling, we compute the signal preserved by pruning ( and sharing ) as $\rho(y, y_p)$ ( and $\rho(y, y_r)$ ) where $\rho$ is the correlation between the two w.r.t the distribution of $x = (x_1, .... x_k)$

\begin{equation}
    \rho(y, y_r) = \frac{Cov(y, y_r)}{\sqrt{Var(y)} \sqrt{Var(y_r)} }
\end{equation}

Assuming that $x_i$ are independent and have the same standard deviation ( i.e inputs are normalized)
\begin{equation}
    Var(y) = k \Bar{\alpha^2} \sigma^2
\end{equation}
where $\Bar{\alpha^2} = \frac{1}{k}(\sum_{i=1}^k \alpha_i^2)$
\begin{equation}
    Var(y_p) = \beta_p^2 \sigma^2
\end{equation}
\begin{equation}
    Var(y_r) = \beta_s^2 k \sigma^2
\end{equation}
\begin{equation}
    Cov(y, y_p) =  Cov( \sum_{i=1}^k  \alpha_i x_i , \beta_p x_1)  = \alpha_1 \beta_p \sigma^2
\end{equation}
\begin{equation}
    Cov(y, y_r) =  Cov( \sum_{i=1}^k  \alpha_i x_i , \beta_s \sum_{i=1}^k x_i)  = \beta_s (\sum_{i=1}^k \alpha_i) \sigma^2 = k \beta_s \Bar{\alpha} \sigma^2 
\end{equation}
where $\Bar{\alpha} = \frac{1}{k}(\sum_{i=1}^k \alpha_i)$

\begin{equation}
    \rho(y, y_p) = \frac{\alpha_1 \beta_p \sigma^2}{\sqrt{k \Bar{\alpha^2} \sigma^2} \sqrt{\beta_p^2 \sigma^2}}
\end{equation}
\begin{equation}
    \rho(y, y_p) = \frac{\alpha_1}{\sqrt{k \Bar{\alpha^2}} }
\end{equation}

\begin{equation}
    \rho(y, y_r) = \frac{ k \beta_s \Bar{\alpha} \sigma^2 }{\sqrt{k \Bar{\alpha^2} \sigma^2} \sqrt{\beta_s^2 k \sigma^2}}
\end{equation}

\begin{equation}
    \rho(y, y_r) = \frac{\Bar{\alpha}}{\sqrt{\Bar{\alpha^2}}}
\end{equation}

Thus, 
\begin{equation}
    \mathbf{E}_{i \leftarrow \{1,...,k\} } (\rho(y, y_p)) = \frac{1}{\sqrt{k}} (\rho(y, y_r))
\end{equation}

Thus the signal is better preserved in parameter sharing. 



==> text/simple_theory_2.tex <==
\clearpage
\section{Theory : Dimensionality reduction analysis on Inner-Products}

Consider two vectors $x$ and $y$ in $R^n$ space. There are two methods to perform dimensoinality reduction 

\begin{enumerate}
    \item Subsample the vector ( making it sparse / pruning ) The transformation is 
    \begin{equation}
        \hat{x} = \sqrt{\frac{n}{m}} Sx 
    \end{equation}
    where S is a $m \times n$ sampling matrix composed of only zeros and ones. Also, each row has exactly one element non-zero. Each column has a maximum of one non-zero.
    \item Projection ( randomly combining the different elements ) In this case, we perform the following transformation
    \begin{equation}
        \hat{x} = R P x
    \end{equation}
    where P is a random permutation matrix and R is a $m \times n$ matrix. R is the random ROAST++ matrix.
\end{enumerate}


Let us look at the inner product preservation in both cases. 
\subsection{pruning}
the estimator of inner products
\begin{equation}
    \langle \hat{x}, \hat{y} \rangle = \frac{n}{m} \sum_{i=1}^n x_i y_i \mathbf{1}(i)
\end{equation}
where $\mathbf{1}(i)$ implies that $i$ is selected.

\begin{equation}
    \mathbf{E}(\langle \hat{x}, \hat{y} \rangle) = \frac{n}{m} \frac{m}{n} \sum_{i=1}^n x_i y_i = \langle x, y \rangle 
\end{equation}

\begin{align}
    (\langle \hat{x}, \hat{y} \rangle)^2 = &  \frac{n^2}{m^2} \left( \sum_{i=1}^n x_i y_i \mathbf{1}(i) \right)^2 \\
    =  & \frac{n^2}{m^2} \left( \sum_{i,j=1}^n x_i y_i x_j y_j \mathbf{1}(i) \mathbf{1}(j) \right) \\
    = & \frac{n^2}{m^2} \left( \sum_{i=1}^n x_i^2 y_i^2 \mathbf{1}(i) 
 + \sum_{i\neq j; 
 i,j=1}^n x_i y_i x_j y_j \mathbf{1}(i) \mathbf{1}(j) \right)
\end{align}

\begin{align}
    \mathbf{E}(\langle \hat{x}, \hat{y} \rangle)^2 &  = \left( \frac{n^2}{m^2} \frac{m}{n} \sum_{i=1}^n  x_i^2 y_i^2 \right) + \left( \frac{n^2}{m^2} \frac{m(m-1}{n(n-1)} \sum_{i\neq j; 
 i,j=1}^n x_i y_i x_j y_j \right) \\
 & = \left( \frac{n}{m} \sum_{i=1}^n  x_i^2 y_i^2 \right) + \left( \frac{n}{m} \frac{(m-1)}{(n-1)} \sum_{i\neq j; 
 i,j=1}^n x_i y_i x_j y_j \right)
\end{align}

Thus, the variance, 

\begin{equation}
    \mathbf{V}(\langle \hat{x}, \hat{y} \rangle) =  \left( \left( \frac{n}{m} - 1 \right) \sum_{i=1}^n  x_i^2 y_i^2 \right) + \left( \left( \frac{1 -1/m}{1-1/n} - 1 \right)  \sum_{i\neq j; 
 i,j=1}^n x_i y_i x_j y_j \right)
\end{equation}


\subsection{Parameter sharing}

the estimator of inner products. Let $h$ be the final position mapping resulting from $P$ and $R$. The signs from $R$ are represented by the function $g$
\begin{equation}
    \langle \hat{x}, \hat{y} \rangle = \sum_{i=1}^m \left( \sum_{j=1}^n x_j g(j) \mathbf{1}(h(j) = i) \right) \left( \sum_{j=1}^n y_j g(j) \mathbf{1}(h(j) = i) \right) 
\end{equation}
where $\mathbf{1}$ is indicator.
The equation can be simplified as,

\begin{equation}
    \langle \hat{x}, \hat{y} \rangle = \sum_{i=1}^m \left( \sum_{j,k=1}^n x_j y_k g(j) g(k) \mathbf{1}(h(j) = i) \mathbf{1}(h(k) = i) \right) 
\end{equation}
which can be further simplified as,

\begin{equation}
    \langle \hat{x}, \hat{y} \rangle = \sum_{i,j=1}^n  x_i y_j g(i) g(j) \mathbf{1}(h(i) = h(j)) 
\end{equation}

\begin{equation}
    \mathbf{E}(\langle \hat{x}, \hat{y} \rangle) = \langle x, y \rangle
\end{equation}

\begin{equation}
    \langle \hat{x}, \hat{y} \rangle^2 = \sum_{a,b,c,d} x_a y_b x_c y_d g(a) g(b) g(c) g(d) \mathbf{1}(h(a) = h(b)) \mathbf{1}(h(c) = h(d))
\end{equation}
Only 4 cases give the non-zero terms in expectations
\begin{itemize}
    \item $a=b=c=d$
    \item $a=b \neq c=d$
    \item $a=c\neq b=d$
    \item $a=d \neq b=c$
\end{itemize}

\begin{align}
    \mathbf{E}(\langle \hat{x}, \hat{y} \rangle^2) & = \sum_{i} x_i^2 y_i^2 \\
    & + \sum_{i\neq j} x_i y_i x_j y_j \\
    & + \sum_{i \neq j} x_i^2 y_j^2 \mathbf{E}(\mathbf{1}(h(i) = h(j))) \\
    & + \sum_{i \neq j} x_i y_i x_j y_j \mathbf{E}(\mathbf{1}(h(i) = h(j)))
\end{align}
Thus variance,
\begin{align}
    \mathbf{V}(\langle \hat{x}, \hat{y} \rangle^2) & = \sum_{i \neq j} x_i^2 y_j^2 \mathbf{E}(\mathbf{1}(h(i) = h(j))) \\
    & + \sum_{i \neq j} x_i y_i x_j y_j \mathbf{E}(\mathbf{1}(h(i) = h(j)))
\end{align}

\begin{equation}
    \mathbf{Pr}(h(i) = h(j) = \textrm{ Pr(i and j in different chunk) Pr( i and j from different chunks collide ) }
\end{equation}
Assming that $m$ divides $n$
\begin{equation}
    \mathbf{Pr}(h(i) = h(j) = \left( 1 - \frac{m-1}{n- 1} \right) \frac{1}{m} 
\end{equation}

\begin{align}
    \mathbf{V}(\langle \hat{x}, \hat{y} \rangle^2) & = \frac{1}{m} \frac{n-m}{n-1} \left( \sum_{i \neq j} x_i^2 y_j^2  + \sum_{i \neq j} x_i y_i x_j y_j \right)
\end{align}

\subsection{Comparison}
As is clear from the two expressions, which method of compression is better depends on the $x$ and $y$ at hand. So in order to get a sense of which method is better on ``average", let us take some interesting distributions from which these points are drawn.

\paragraph{Equal strength components}
Let $x_i, y_i$ are i.i.d, mean zero and standard-deviation $\sigma$ ( for example,  $\mathcal{N}(0, \sigma^2 I)$ ). We will denote statistics w.r.t these data distributions with a subscript $\mathcal{D}$
\begin{equation}
\mathbf{E}_{D} (\mathbf{V}_{prun}(\langle \hat{x}, \hat{y} \rangle) ) = \left(\frac{n}{m} - 1 \right) n \sigma^4    
\end{equation}
\begin{equation}
\mathbf{E}_{D} (\mathbf{V}_{roast++}(\langle \hat{x}, \hat{y} \rangle) ) = \frac{1}{m} \frac{n-m}{n-1} n(n-1) \sigma^4 = \left( \frac{n}{m} - 1 \right) n \sigma^4    
\end{equation}

Thus, under equal strength components, in expectation over the data, both methods perform equally well.

\paragraph{Unequal strengths / Sparsity of signals}
WLOG, let $x_1$ be the strongest signal and the signal strength of $x_i$ reduce with increasing $i$. To model this, we will do the following. Let all $x_is$ be zero-mean and their variances be defined as
\begin{equation}
    \mathbf{V}_{\mathbf{D}}(x_i) = \sigma^2 e^{-ti} \;\; \forall i \in \{0,...,n{-}1\}
\end{equation}
where $t>0$ is a temperature parameter to control the power-law of variances.
\begin{equation}
\mathbf{E}_{D} (\mathbf{V}_{prun}(\langle \hat{x}, \hat{y} \rangle) ) = \left(\frac{n}{m} - 1 \right) \sigma^4 \sum_{i=0}^{n-1} e^{-2ti} = \left(\frac{n}{m} - 1 \right) \sigma^4 \left(  \frac{1-e^{-2tn}}{1 - e^{-2t}}\right)    
\end{equation}

\begin{align}
\mathbf{E}_{D} (\mathbf{V}_{roast++} 
 & (\langle \hat{x}, \hat{y} \rangle) )  = \frac{1}{m} \frac{n-m}{n-1} \sigma^4 \left(  \sum_{i\neq j} e^{-t(i+j)}\right)
\end{align}

\begin{align}
    \left(  \sum_{i\neq j} e^{-t(i+j)}\right) = \left(  \sum_{i=0}^{n-1} e^{-ti} \right) \left(  \sum_{j=0}^{n-1} e^{-tj} \right) - \left(  \sum_{i} e^{-2ti} \right)
\end{align}
\begin{align}
    \left(  \sum_{i\neq j} e^{-t(i+j)}\right) = \left(  \sum_{i=0}^{n-1} e^{-ti} \right)^2 - \left(  \sum_{i} e^{-2ti} \right)
\end{align}

\begin{align}
    \left(  \sum_{i\neq j} e^{-t(i+j)}\right) = \left(\frac{1 - e^{-tn}}{1 - e^{-t}} \right)^2 - \frac{1 - e^{-2nt}}{1 - e^{-2t}}
\end{align}

\begin{align}
\mathbf{E}_{D} (\mathbf{V}_{roast++} 
 & (\langle \hat{x}, \hat{y} \rangle) )  = \frac{1}{n-1} \frac{n-m}{m} \sigma^4 \left(  \left(\frac{1 - e^{-tn}}{1 - e^{-t}} \right)^2 - \frac{1 - e^{-2nt}}{1 - e^{-2t}}   \right)
\end{align}

Consdier
\begin{equation}
    \frac{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{roast++})}{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{prune})} = \frac{1}{n-1} \frac{\left(  \left(\frac{1 - e^{-tn}}{1 - e^{-t}} \right)^2 - \frac{1 - e^{-2nt}}{1 - e^{-2t}}   \right)}{\left(  \frac{1-e^{-2tn}}{1 - e^{-2t}}\right)  }
\end{equation}
\begin{equation}
    \frac{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{roast++})}{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{prune})} = \frac{1}{n-1} \left( \frac{  \left(\frac{1 - e^{-tn}}{1 - e^{-t}} \right)^2 }{\left(  \frac{1-e^{-2tn}}{1 - e^{-2t}}\right) }  -1 \right)
\end{equation}
It can be seen by plotting the function that the function obtains maximum at $t=0$ and reduces as $t$ increases. 



\begin{equation}
    \rho(\textrm{ratio}) = \frac{  \left(\frac{1 - e^{-tn}}{1 - e^{-t}} \right)^2 }{\left(  \frac{1-e^{-2tn}}{1 - e^{-2t}}\right)} \frac{1}{n}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[scale=0.15]{theory-images/ratio_plot.png}
    \caption{Plot of $\rho$ for different values of $n$}
    \label{fig:enter-label}
\end{figure}
Max value of the function at $t=0$ is $n$. Thus, 

\begin{equation}
    \frac{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{roast++})}{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{prune})} = \frac{1}{n-1} \left( \frac{  \left(\frac{1 - e^{-tn}}{1 - e^{-t}} \right)^2 }{\left(  \frac{1-e^{-2tn}}{1 - e^{-2t}}\right) }  -1 \right) \leq 1
\end{equation}
where equality happens at $t=0$

Thus 
\begin{equation}
    \frac{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{roast++})}{\mathbf{E}_{\mathcal(D)}(\mathbf{V}_{prune})} \leq 1
\end{equation}
with equality happens at $t=0$. Thus, at any $t>0$ i.e. even a slightly unbalanced signal strengths, pruning is at a disadvantage to parameter sharing via roast++.

\section{Theory : Dimensionality reduction analysis on Norms}
For norms (precisely square of norm) we can just use $x=y$ in the previous analysis
\begin{equation}
    \mathbf{V}_{prune}(\langle \hat{x}, \hat{x} \rangle) =  \left( \left( \frac{n}{m} - 1 \right) \sum_{i=1}^n  x_i^4 \right) + \left( \left( \frac{1 -1/m}{1-1/n} - 1 \right)  \sum_{i\neq j; 
 i,j=1}^n x_i^2 x_j^2 \right)
\end{equation}

\begin{align}
    \mathbf{V}_{\roastpp}(\langle \hat{x}, \hat{x} \rangle^2) & = \frac{2}{m} \frac{n-m}{n-1} \left( \sum_{i \neq j} x_i^2 x_j^2 \right)
\end{align}


\subsection{Comparison : Equal strength}
If one method is better than other for a given $x$ at preserving $||x||^2$, then for all $\lambda \in R$, the same method is better for $\lambda x$. We can consider normal distribution WLOG as we just need a radially symmetric distribution.

\begin{align}
    \mathbf{E}_D (\mathbf{V}_{prune}(\langle \hat{x}, \hat{x} \rangle)) & =  \left( \left( \frac{n}{m} - 1 \right) 3 n \sigma^4 \right) + \left( \left( \frac{1 -1/m}{1-1/n} - 1 \right)  n(n-1) \sigma^4 \right) \\
    & = \sigma^4 \left( \frac{3n(n-m)}{m} + \left( 
\frac{m-n}{m(n-1)} n(n-1) \right) \right) \\
& = \sigma^4 \left( \frac{3n(n-m)}{m} + \left( 
\frac{m-n}{m} n \right) \right)\\
& = \frac{2n(n-m)}{m} \sigma^4 
\end{align}


\begin{align}
    \mathbf{E}_D(\mathbf{V}_{\roastpp}(\langle \hat{x}, \hat{x} \rangle^2)) & = \frac{2}{m} \frac{n-m}{n-1} n(n-1) \sigma^4 = \frac{2n(n-m)}{m} \sigma^4
\end{align}
Thus, under equal strength (data drawn randomly radially symmetrically) both methods are equivalent ( one is better equal number of times)

\subsection{Comparison : Unequal strength}
WLOG, let $x_1$ be the strongest signal and the signal strength of $x_i$ reduce with increasing $i$. To model this, we will do the following. Let all $x_is$ be zero-mean and their variances be defined as
\begin{equation}
    \mathbf{V}_{\mathbf{D}}(x_i) = \sigma^2 e^{-ti} \;\; \forall i \in \{0,...,n{-}1\}
\end{equation}

\begin{equation}
    \mathbf{E}_D(\mathbf{V}_{prune}(\langle \hat{x}, \hat{x} \rangle)) =  \left( \frac{n-m}{m}  \sum_{i=1}^n  3 e^{-2ti} \sigma^4 \right) + \left( \frac{m-n}{m(n-1)}   \sum_{i\neq j} \sigma^4 e^{-t(i+j)} \right)
\end{equation}

\begin{align}
    \mathbf{E}_D(\mathbf{V}_{\roastpp}(\langle \hat{x}, \hat{x} \rangle^2)) & = \frac{2}{m} \frac{n-m}{n-1} \left( \sum_{i \neq j} \sigma^4 e^{-t(i+j)} \right)
\end{align}

\begin{align}
\frac{\mathbf{E}_D(\mathbf{V}_{\roastpp} (||x||^2))  }{\mathbf{E}_D(\mathbf{V}_{prune} (||x||^2))} = \frac{ 2 \sum_{i \neq j} e^{-t(i+j)}}{3 (n-1) \sum_{i=1}^n e^{-2ti} - \sum_{i \neq j}  e^{-t(i+j)} }
\end{align}

\begin{align}
\frac{\mathbf{E}_D(\mathbf{V}_{\roastpp} (||x||^2))  }{\mathbf{E}_D(\mathbf{V}_{prune} (||x||^2))} = \frac{ 2}{3 \left( \frac{(n-1) \sum_{i=1}^n e^{-2ti}}{\sum_{i \neq j} e^{-t(i+j)}} \right) - 1 }
\end{align}

\begin{align}
\frac{\mathbf{E}_D(\mathbf{V}_{\roastpp} (||x||^2))  }{\mathbf{E}_D(\mathbf{V}_{prune} (||x||^2))} = \frac{ 2}{3 \left( \frac{(n-1)}{ \frac{(\sum_{i} e^{-ti})^2}{\sum_{i} e^{-2ti}} - 1} \right) - 1 }
\end{align}
Note that 
\begin{equation}
\frac{(\sum_{i} e^{-ti})^2}{\sum_{i} e^{-2ti}}  \leq n   
\end{equation}

Thus,
\begin{align}
\frac{\mathbf{E}_D(\mathbf{V}_{\roastpp} (||x||^2))  }{\mathbf{E}_D(\mathbf{V}_{prune} (||x||^2))} \leq 1
\end{align}
with equality only when $t=0$


\section{Theory : Analysis of linear models under Pruning and ROAST++}
Consider the following features $x_1, x_2, ... x_n$ such that,
\begin{equation}
    Var(x_i) = V(x_i) = \sigma_x^2 \; \forall i  \qquad \textrm{ and } \qquad Cov(x_i, x_j) = C(x_i, x_j) = 0 \; \forall i \neq j
\end{equation}

\paragraph{Pruning.}
\begin{align}
    Res(\hat{y}) = Var( y - \sum_i \alpha_i \mathbf{1}(i) x_i) 
\end{align}
\begin{align}
    Res(\hat{y}) = V(y) + \sum_i \alpha_i^2 \mathbf{1}(i) V(x_i) - 2 \sum_i \alpha_i \mathbf{1}(i) C(y,x_i)
\end{align}

Minimizing the residual, we get,
\begin{equation}
    \mathbf{1}(i) \alpha_i = \frac{C(y, x_i)}{\sigma_x^2} 
\end{equation}

\begin{align}
    Res(\hat{y}) = V(y) - \sum_i \frac{C(y,x_i)^2}{\sigma_x^2} \mathbf{1}(i)
\end{align}


Let $\rho(i) = \frac{Cov(y, x_i)}{\sigma_x}$

\begin{align}
    Res(\hat{y}) = V(y) - \sum_i  \mathbf{1}(i) \rho(i)^2
\end{align}

\paragraph{ROAST++}
\begin{align}
    Res(\hat{y}) = Var\left( y - \sum_{j=1}^m \alpha_j \sum_i \mathbf{1}(i,j)g_i x_i\right) 
\end{align}
\begin{align}
    Res(\hat{y}) = V(y) + \sum_j \left(\alpha_j^2 V\left(\sum_i \mathbf{1}(i,j)g_i x_i\right) \right) - 2 \sum_j \alpha_j (i,j) C(y, \sum_i \mathbf{1}(i,j) g_ix_i)
\end{align}

Using the same analysis,
\begin{equation}
    \alpha_j = \frac{C(y, \sum_i \mathbf{1}(i,j) g_ix_i )}{V(\sum_i \mathbf{1}(i,j) g_ix_i)} = \frac{\sum_i \mathbf{1}(i,j) g_i C(y,x_i) }{k \sigma_x^2}
\end{equation}

\begin{align}
    Res(\hat{y}) = V(y) - \sum_j  \frac{C(y, \sum_i \mathbf{1}(i,j) g_i x_i)^2}{V(\sum_i \mathbf{1}(i,j) g_i x_i)}
\end{align}


Let $\rho(i) = \frac{Cov(y, x_i)}{\sigma_x}$

\begin{align}
    Res(\hat{y}) = V(y) - \sum_j  \frac{(\sum_i \mathbf{1}(i,j) \rho(i))^2}{k}
\end{align}

\begin{align}
    Res(\hat{y}) = V(y) - \sum_j  (\sum_i \frac{\mathbf{1}(i,j)g_i}{\sqrt{k}} \rho(i))^2
\end{align}

So the residual is minimized based on how large is the second term.

\subsection{Comparison}
It is clear from the above two analysis that essential question is about norm-preservation of the vector of $(\rho(1), \rho(2), \rho(3) , .... , \rho(n)$ under sampling and roast++ sketching.


